Towards Bidirectional Protection in Federated Learning

Prior efforts in enhancing federated learning (FL) security fall into two categories. At one end of the spectrum, some work uses secure aggregation techniques to hide the individual client's updates and only reveal the aggregated global update to a malicious server that strives to infer the clients' privacy from their updates. At the other end of the spectrum, some work uses Byzantine-robust FL protocols to suppress the influence of malicious clients' updates. We present a federated learning protocol F2ED-LEARNING, which, for the first time, offers bidirectional defense to simultaneously combat against the malicious centralized server and Byzantine malicious clients. To defend against Byzantine malicious clients, F2ED-LEARNING provides dimension-free estimation error by employing and calibrating a well-studied robust mean estimator FilterL2. F2ED-LEARNING also leverages secure aggregation to protect clients from a malicious server. One key challenge of F2ED-LEARNING is to address the incompatibility between FilterL2 and secure aggregation schemes. Concretely, FilterL2 has to check the individual updates from clients whereas secure aggregation hides those updates from the malicious server. To this end, we propose a practical and highly effective solution to split the clients into shards, where F2ED-LEARNING securely aggregates each shard's update and launches FilterL2 on updates from different shards. The evaluation shows that F2ED-LEARNING consistently achieves optimal or close-to-optimal performance and outperforms five secure FL protocols under five popular attacks.

==> app_eval.tex <==
% \section{Other Attacks}
% \label{sec:attack}

\section{Model Replacement Attack}
\label{sec:attack}

In this section, we focus on the backdoor attack introduced in~\cite{bagdasaryan2020backdoor}, namely model replacement attack.
%
Similar to MPA, we use Attack Success Rate as the metric to measure the robustness of an estimator.
%
The results are included in Figure~\ref{fig:backdoor}.

\captionsetup{font={footnotesize}}
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \resizebox{\textwidth}{!}{\input{figs/main/orig/INFIMNIST/backdoor}}
    \caption{INFIMNIST under Model Replacement Attack~\cite{bagdasaryan2020backdoor}.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \resizebox{\textwidth}{!}{\input{figs/main/orig/fashionMNIST/backdoor}}
    \caption{FashionMNIST under Model Replacement Attack~\cite{bagdasaryan2020backdoor}.}
    \end{subfigure}
    \caption{\lun{fill in this}}
    \label{fig:backdoor}
\end{figure}

% \subsection{DBA}

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \\\answerYes{The contribution and scope of this paper is accurately summarized in abstract and introduction.}
  \item Did you describe the limitations of your work?
    \\\answerYes{We discuss on the limitations and promising future directions in \S~\ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \\\answerYes{We discuss the influence of shard size in \S~\ref{sec:eval-results} and Appendix~\ref{sec:eval-shardsize}, we deem that too small shards number will weaken the robustness of \system and provide an opportunity for malicious clients to conduct poisoning attack. While too large shards number will sacrifice the security of \system, which will provide an opportunity for malicious server to conduct inference attack. We also talk about the optimal choice of shard size in Appendix~\ref{sec:eval-shardsize}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \\\answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \\\answerYes{The threat model which assumes the capability of malicious clients or server is elaborated in \S~\ref{sec:threat-model}. All the assumptions required for the theoretical results are elaborated in \S~\ref{sec:system} or in the corresponding proof in Appendix~\ref{sec:proof-corollary1}, Appendix~\ref{sec:proof-corollary2}, and Appendix~\ref{sec:proof-corollary3}.}
  \item Did you include complete proofs of all theoretical results?
    \\\answerYes{All proofs are included in \S~\ref{sec:system} and Appendix~\ref{sec:proof-corollary1}, Appendix~\ref{sec:proof-corollary2}, and Appendix~\ref{sec:proof-corollary3}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \\\answerYes{All the code, data, and instructions on how to reproduce the experimental results can be found in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \\\answerYes{All the evaluation setup details are elaborated in \S~\ref{sec:evaluation} and Appendix~\ref{sec:eval-setup-append}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \\\answerNo{We clarify that we do not provide the error bars whose reasons are threefold as
follows. First, we note that all the initial states of the models are the same
and all the experiments use the same random seed. Similarly, all
hyper-parameters and other settings are the same. Hence, we deem that the
comparison among the estimators is fair. Second, previous defense methods like
Krum~\cite{blanchard2017machine}, Bulyan~\cite{mhamdi2018hidden}, and Trimmed
Mean~\cite{yin2018byzantine} and previous attacks like
MPA~\cite{bhagoji2019analyzing}, MRA~\cite{bagdasaryan2020backdoor},
DBA~\cite{xie2019dba} do not report the error bars in their evaluation. Besides,
KA~\cite{fang2019local} and TMA~\cite{fang2019local} omit the error bars, and as
disclosed in their papers, the observed variances are \textit{very small}.
Hence, we deem that our evaluation setting is aligned with these relevant
previous works. Third, some estimators adopted in our evaluation, e.g.,
BulyanKrum and BulyanTrimmedMean, are highly computation-intensive: we report
that running one experiment under a single attack can take over 24 hours, and
therefore, reporting error bars is generally beyond our computation power.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \\\answerYes{They are included in Appendix~\ref{sec:eval-setup-append}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \\\answerYes{We have cited all the creators of the algorithms and datasets we use in this paper.}
  \item Did you mention the license of the assets?
    \\\answerYes{We mention the license of dataset in Appendix~\ref{sec:eval-setup-append}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \\\answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \\\answerNA{The datasets or algorithms we use are publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \\\answerNA{The datasets used in this paper don't contain personally identifiable information or offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \\\answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \\\answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \\\answerNA{}
\end{enumerate}

\end{enumerate}


==> corollary1.tex <==
\section{Proof of Corollary~\ref{cor:sec}}
\label{sec:cor1}

\begin{proof}
Corollary~\ref{cor:sec} is equivalent to the following lemma.

\begin{lemma}[Lemma 6.1 in~\cite{bonawitz2017practical}]
Given the number of the shards $p$, the parameter size $d$, the group size $q$, and the updates $\textbf{g}^{H_i}$ where $\forall i\in[p], \textbf{g}^{H_i}\in \mathbb{Z}^d_q$, we have 
\begin{equation*}
\begin{split}
    &\{\{\textbf{u}_{ij}\overset{\$}{\leftarrow}\mathbb{Z}_q^d\}_{i<j}, \textbf{u}_{ij}\coloneqq
    -\textbf{u}_{ji},\\ &\forall i>j: \{\textbf{g}^{H_i}+\sum_{j\in[p]\slash i}\textbf{u}_{ij} \pmod{q}\}_{i\in[p]}\}
    \\ \equiv &\{\{\textbf{v}_i\overset{\$}{\leftarrow}\mathbb{Z}_q^d\}_{i\in[p]}\}~s.t.~ \sum_{i\in[p]}\textbf{v}_i=\sum_{i\in[p]}\textbf{g}^{H_i} \pmod{q}: \{\textbf{v}_{i}\}_{i\in[q]}\}
\end{split}
\end{equation*}
where "$\equiv$" denotes that the distributions are identical.
\label{lem:sec}
\end{lemma}

We prove the above lemma with induction on $n$.

\paragraph{Base case:} When $n=2$, the first elements in the RHS of two distributions are both uniformly random.
%
The second element is the sum minus the first element.
%
Thus the distributions are identical.

\paragraph{Inductive Hypothesis:}
We assume that when $n=k$, the two distributions are identical.

\paragraph{Inductive Step:}
If we ignore all the randomness from and for client $k+1$, according to the inductive hypothesis, the distributions of the first $k$ clients are identical.
%
Hence, after adding two independently uniformly random values, the distributions are still identical.
%
The value for the $k+1^{th}$ client the the sum minus $k$ uniformly random values.
%
Thus, the two distributions are still identical.

\end{proof}

==> corollary2.tex <==
\section{Proof of Corollary~\ref{cor:robust}}
\label{sec:cor2}

\begin{proof}
In the following analysis, we assume that the updates from the shards follow an i.i.d. distribution.
%
The reasonableness of the assumption is further discussed in Section~\ref{sec:iid}.

The fraction of malicious shards is bounded by the worst case where each malicious client is exclusively assigned to different shards: $\epsilon'\leq \frac{\epsilon n}{p}\leq \frac{1}{12}$.
%
Given the assumption above, we have satisfied all the requirements in Theorem~\ref{thm:filterl2}.
%
Hence, \system provides a mean estimation with dimension-free error as long as $12\epsilon n < p$.

\end{proof}

==> corollary3.tex <==
\section{Proof of Corollary~\ref{cor:clt}}
\label{sec:cor3}

\begin{proof}

By reorganizing Equation~\ref{eq:clt}, we have $\frac{1}{|H|}\sum_{i\in H}g_i\overset{d}{\rightarrow} N(\frac{1}{|H|}\sum_{i\in H}\mu_{\phi(i)}, \frac{s_H^2}{|H|^2})$.
%
Given the multinomial distribution $\Phi$,
\begin{itemize}
    \item $\mathbb{E}[\frac{\sum_{i\in H}\mu_{\phi(i)}}{|H|}]=\sum_{i\in[k]}\Phi(x=i)\mu_i=\bar{\mu}$,
    $\mathbb{V}[\frac{\sum_{i\in H}\mu_{\phi(i)}}{|H|}]=\frac{\sum_{i\in[k]}\Phi(x=i)(\mu_i-\bar{\mu})^2}{|H|}=\frac{\sigma_{\mathbb{E}}^2}{|H|}$
    \item $\mathbb{E}[\frac{s_H^2}{|H|}]=\sum_{x\in[k]}\Phi(x=i)\sigma_i^2=\bar{\sigma}^2$, $\mathbb{V}[\frac{s_H^2}{|H|}]=\frac{\sum_{x\in[k]}\Phi(x=i)(\sigma_i^2-\bar{\sigma}^2)^2}{|H|}=\frac{\sigma_{\mathbb{V}}^2}{|H|}$
\end{itemize}
%
Thus, when $|H|\rightarrow\infty$, $\frac{\sum_{i\in H}\mu_{\phi(i)}}{|H|}\rightarrow\bar{\mu}$, $\frac{s_H^2}{|H|^2}\rightarrow\frac{\bar{\sigma}^2}{|H|}$.
\end{proof}

==> fig4.tex <==
\begin{figure*}[htbp]
     \centering
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/orig/INFIMNIST/withoutattack}}
         \caption{MNIST non-attack.}
         \label{fig:mnist_noattack3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/orig/INFIMNIST/krum}}
         \caption{MNIST under KA.}
         \label{fig:mnist_krum3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/orig/INFIMNIST/trimmedmean}}
         \caption{MNIST under TMA.}
         \label{fig:mnist_trimmedmean3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/orig/INFIMNIST/modelpoisoning}}
         \caption{MNIST under MPA.}
         \label{fig:mnist_modelpoisoning3}
     \end{subfigure}
     
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/orig/INFIMNIST/backdoor}}
         \caption{MNIST under MRA.}
         \label{fig:mnist_backdoor}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/orig/INFIMNIST/dba}}
         \caption{MNIST under DBA.}
         \label{fig:mnist_dba}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/withoutattack}}
    %      \caption{FashionMNIST non-attack.}
    %      \label{fig:fashionmnist_noattack2}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/krum}}
    %      \caption{FashionMNIST under KA.}
    %      \label{fig:fashionmnist_krum2}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/trimmedmean}}
    %      \caption{FashionMNIST under TMA.}
    %      \label{fig:fashionmnist_trimmedmean2}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/modelpoisoning}}
    %      \caption{FashionMNIST under MPA.}
    %      \label{fig:fashionmnist_modelpoisoning2}
    %  \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \raisebox{\height}{\resizebox{\textwidth}{!}{\input{figs/main/legend}}}
     \end{subfigure}
    \hfill
    \caption{Attack performance under different estimators with non-i.i.d. data.}
    \label{fig:f4}
    \vspace{-10pt}
\end{figure*}

==> fig5.tex <==
\begin{figure*}[htbp]
     \centering
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/shard/INFIMNIST/withoutattack}}
         \caption{MNIST non-attack.}
         \label{fig:mnist_noattack4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/shard/INFIMNIST/krum}}
         \caption{MNIST under KA.}
         \label{fig:mnist_krum4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/shard/INFIMNIST/trimmedmean}}
         \caption{MNIST under TMA.}
         \label{fig:mnist_trimmedmean4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/shard/INFIMNIST/modelpoisoning}}
         \caption{MNIST under MPA.}
         \label{fig:mnist_modelpoisoning4}
     \end{subfigure}
     
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/shard/INFIMNIST/backdoor}}
         \caption{MNIST under MRA.}
         \label{fig:mnist_modelpoisoning4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\figwidth}
         \centering
         \resizebox{\textwidth}{!}{\input{figs/hetero/shard/INFIMNIST/dba}}
         \caption{MNIST under DBA.}
         \label{fig:mnist_modelpoisoning4}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/withoutattack}}
    %      \caption{FashionMNIST non-attack.}
    %      \label{fig:fashionmnist_noattack2}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/krum}}
    %      \caption{FashionMNIST under KA.}
    %      \label{fig:fashionmnist_krum2}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/trimmedmean}}
    %      \caption{FashionMNIST under TMA.}
    %      \label{fig:fashionmnist_trimmedmean2}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{\figwidth}
    %      \centering
    %      \resizebox{\textwidth}{!}{\input{figs/hetero/shard/fashionMNIST/modelpoisoning}}
    %      \caption{FashionMNIST under MPA.}
    %      \label{fig:fashionmnist_modelpoisoning2}
    %  \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \raisebox{\height}{\resizebox{\textwidth}{!}{\input{figs/main/legend2}}}
     \end{subfigure}
    \hfill
    \vspace{-5pt}
    \caption{Attack performance under different estimators with sharded secure aggregation and non-i.i.d. data.}
    \label{fig:f5}
    \vspace{-10pt}
\end{figure*}

==> figs/main/legend_for_fig6.tex <==
\newenvironment{customlegend}[1][]{%
    \begingroup
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\begin{tikzpicture}
\begin{customlegend}[legend columns=5,legend style={align=left,draw=none,column sep=2ex},
        legend entries={\textsc{10 shards},\textsc{20 shards}, \textsc{25 shards},\textsc{50 shards},\textsc{100 shards}}]
        % \addlegendimage{mark=none,black,line width=1.6pt}
        \addlegendimage{mark=none,dashed,red,line width=1.6pt}
        \addlegendimage{mark=none,dashed,blue,line width=1.6pt}
        \addlegendimage{mark=none,dashed,brown,line width=1.6pt}
        \addlegendimage{mark=none,dashed,darkgreen,line width=1.6pt}
        \addlegendimage{mark=none,dashed,orange,line width=1.6pt}
        \end{customlegend}
\end{tikzpicture}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> prelim.tex <==
\section{Preliminaries: Robust Mean Estimation \& Secure Aggregation}
\label{sec:prelim}
%
In this section, we review the two main building blocks: robust mean estimation and secure aggregation in \system.

\lun{iterate over this}
\subsection{Robust Mean Estimation.} 
%
The core step in federated learning is to aggregate the individual updates from the clients.
%
The most commonly used aggregation is to average all the updates.
%
Given the threat model that some clients might be malicious, we want to estimate the mean value as close as to the true mean value without the malicious updates. 
%
There are a spectrum of works focusing on addressing the problem in the such as Krum~\cite{blanchard2017machine} and Bulyan~\cite{mhamdi2018hidden}.
%
However, all the known estimators' estimation error grows proportionally with $\sqrt{d}$ where $d$ is the parameter size of the model.
%
Such error is unacceptable in federated learning since the model size is typically tens of thousands to hundreds of thousands.

Actually, the problem is well studied in statistics under the name ``robust mean estimation'' and there already exist several robust mean estimators with dimension-free estimation error~(\cite{diakonikolas2019robust,charikar2017learning,steinhardt2018robust,cheng2019high,dong2019quantum}).
%
We present a representative aggregator namely \agg here.
%
\begin{algorithm}%[H]
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Fn}{Function}{:}{\KwRet}
\SetAlgoLined
\KwIn{$\textbf{x}_1, \cdots, \textbf{x}_n\in\mathbb{R}^d$, $\eta>1$}
Let $c_1, \cdots, c_n=1$\;
$\hat{\boldsymbol{\mu}}_c=(\sum_{i=1}^nc_i\textbf{x}_i)/(\sum_{i=1}^nc_i)$\;
$\hat{\boldsymbol{\Sigma}}_c=(\sum_{i=1}^nc_i(\textbf{x}_i-\hat{\mu}_c)(\textbf{x}_i-\hat{\mu}_c)^\top)/(\sum_{i=1}^nc_i)$\;
Let $v$ be the maximum eigenvector of $\hat{\boldsymbol{\Sigma}}_c$, and let $\hat{\sigma}_c^2=\textbf{v}^\top\hat{\boldsymbol{\Sigma}}_c\textbf{v}$\;
\lIf{$\hat{\sigma}_c^2\leq \eta\sigma^2$}{return $\hat{\boldsymbol{\mu}}_c$}
\lElse{let $\tau=\langle \textbf{x}_i-\hat{\boldsymbol{\mu}}_c\rangle^2$, and update $c_i\leftarrow c_i\cdot (1-\tau_i/\tau_{\max})$, where $\tau_{\max}=\max_i\tau_i$}
Go back to line 2\;
\caption{\agg: dimension-free robust mean estimation~(\cite{diakonikolas2019robust}).}
\label{alg:filterl2}
\end{algorithm}

As mentioned, \agg provides dimension-free error rate formally presented as follow.
%
\begin{theorem}
Let $\mathcal{D}$ be the honest dataset and $\mathcal{D}^{*}$ be the contaminated version of $\mathcal{D}$ by inserting arbitrary samples.
%
Suppose that $|\mathcal{D}^{*}|\leq |\mathcal{D}|/(1-\epsilon)$, and further suppose that $\textsc{Mean}[\mathcal{D}]=\boldsymbol{\mu}$ and $\|\textsc{Cov}[\mathcal{D}]\|_{op}\leq\sigma^2$. %
Then given $\mathcal{D}^*$, Algorithm~\ref{alg:filterl2} outputs $\hat{\boldsymbol{\mu}}$ s.t. $\|\hat{\boldsymbol{\mu}}-\boldsymbol{\mu}\|_2=\mathcal{O}(\sigma\sqrt{\epsilon})$ using $\textsc{poly}(n,d)$ time.
%
% $\textsc{poly}(n,d)$ that outputs $q$ with $\textsc{TV}(p^{*},q)\leq \epsilon$ and $\|\textsc{Cov}_q[X]\|\leq \mathcal{O}(\sigma^2)$.
%
% In particular, $\|\mu(p^{*})-\mu(q)\|_2=\mathcal{O}(\sigma\sqrt{\epsilon})$.
\label{thm:filterl2}
\end{theorem}

\subsection{Secure Aggregation.} 
%
Secure aggregation is a cryptographic technique developed by~\cite{bonawitz2017practical} to defend against a semi-honest server in federated learning.
%
In particular, secure aggregation allows the server to access the averaged update but prevents it from seeing individual updates from clients.
%
Thus, the server cannot launch inference attacks on the individual updates.

To better demonstrate \system, we give a high-level context on how secure aggregation works.
%
As the first step, each client generates random values for all the other clients and send each value to the corresponding client.
%
After receiving all the random values from other clients, each client sums up the received values and subtracts the values generated by itself to produce a random mask.
%
It is clear that all the masks sum up to zero.
%
Then each client blind its update with the random mask and send the blinded update to the server.
%
As the last step, the server sums up all the updates.
%
Obviously, all the masks cancel out during aggregation and the server receives the plaintext sum.

==> proof-lemma1.tex <==
\section{Proof of Lemma~\ref{lem:sec}}
\label{sec:proof-lemma1}

\noindent\textbf{Lemma~\ref{lem:sec}} (Lemma 6.1 in~\cite{bonawitz2017practical}). 
Given the number of the shards $p$, the parameter size $d$, the group size $q$, and the updates $\textbf{g}^{H_i}$ where $\forall i\in[p], \textbf{g}^{H_i}\in \mathbb{Z}^d_q$, we have 
\begin{equation*}
\begin{split}
    &\{\{\textbf{u}_{ij}\overset{\$}{\leftarrow}\mathbb{Z}_q^d\}_{i<j}, \textbf{u}_{ij}\coloneqq -\textbf{u}_{ji} \; \forall i>j \quad : \{\textbf{g}^{H_i}+\sum_{j\in[p]\slash i}\textbf{u}_{ij} \pmod{q}\}_{i\in[p]}\}
    \\ \equiv &\{\{\textbf{v}_i\overset{\$}{\leftarrow}\mathbb{Z}_q^d\}_{i\in[p]}~s.t.~ \sum_{i\in[p]}\textbf{v}_i=\sum_{i\in[p]}\textbf{g}^{H_i} \pmod{q} \quad : \{\textbf{v}_{i}\}_{i\in[q]}\}
\end{split}
\end{equation*}
where "$\equiv$" denotes that the distributions are identical.


\begin{proof}
We prove Lemma~\ref{lem:sec} with induction on $n$.

\noindent\textbf{Base case:} When $n=2$, the first elements of two distributions are both uniformly random.
%
The second element is the sum minus of the corresponding first element.
%
Thus the distributions are identical.

\noindent\textbf{Inductive Hypothesis:}
When $n=k$, the lemma holds.

\noindent\textbf{Inductive Step:}
% If we ignore all the randomness from and for client $k+1$, 
According to the inductive hypothesis, the left and right distributions of the first $k$ clients are indistinguishable.
%
We follow the protocol to generate the left transcript when the $(k+1)^{th}$ client is added to the shard.
%
To deal with the right-hand-side transcript, we first add the same randomness as left-hand-side to the first $k$ updates and then subtract them from the total sum to get the $(k+1)^{th}$ update.
%
It is easy to prove that the first $k$ updates on the left and right follow the same uniformly random distribution and the $(k+1)^{th}$ update is the difference between the total sum and the sum of the first $k$ updates.
%
Hence, the left and right transcripts are indistinguishable.
% To add the $(k+1)^{th}$ client to the left-hand-side distribution, we follow the protocol to add randomness to the first $k$ clients.
%
% To keep the indistinguishability, we add the same randomness to the right-hand-side distribution. 
% %
% For the left-hand-side, we follow the protocol to generate the $(k+1)^{th}$ update while for the right-hand-side, we subtract the first $k$ updates from the total sum to generate the $k^{th}$ update.
% %
% It is easy to prove that the left-hand-side distribution 
% For the right-hand-side distribution, we subtract 
% Hence, after adding two independently uniformly random values, the distributions are still identical.
% %
% The value for the $k+1^{th}$ client is the sum minus $k$ uniformly random values.
% %
% Thus, the two distributions are still identical.

\end{proof}

==> sec_agg.tex <==
\section{Sharded Secure Aggregation}

\begin{algorithm}%[H]
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Fn}{Function}{:}{\KwRet}
\SetAlgoLined
% \KwIn{$\textbf{g}_1, \cdots, \textbf{g}_m\in\mathbb{R}^d$}
The server randomly partitions $[m]$ into $r$ subsets $\{\mathbb{S}_i\}_{i\in[r]}$, $|\mathbb{S}_i|=m/r$\;
\For{$i\in[r]$}{
    \For{$j\in\mathbb{S}_i$}{
        \For{$k\in\mathbb{S}_i-j$}{
            Client $j$ generates random mask $u_{jk}$ and sends the mask to client $k$\;
        }
    }
}
\For{$i\in[m]$}{
    Client $i$ masks the gradient with its own and received randomness $\hat{\textbf{g}}_i=\textbf{g}_i + \sum \textbf{u}_{ik} - \sum \textbf{u}_{ki}$\;
    Client $i$ uploads $\hat{\textbf{g}}_i$ to the server
}
Server computes sharded average $\forall i\in[r], \bar{\textbf{g}}_i=\frac{1}{n}\sum_{j\in\mathbb{S}_i} \hat{\textbf{g}}_j$
\caption{Sharded Secure Aggregation.}
\label{alg:sharded}
\end{algorithm}


